Tracking Multiple Vehicles Using a Variational Radar Model

High-resolution radar sensors are able to resolve multiple detections per object and therefore provide valuable information for vehicle environment perception. For instance, multiple detections allow to infer the size of an object or to more precisely measure the object's motion. Yet, the increased amount of data raises the demands on tracking modules: measurement models that are able to process multiple detections for an object are necessary and measurement-to-object associations become more complex. This paper presents a new variational radar model for tracking vehicles using radar detections and demonstrates how this model can be incorporated into a Random-Finite-Set-based multi-object filter. The measurement model is learned from actual data using variational Gaussian mixtures and avoids excessive manual engineering. In combination with the multiobject tracker, the entire process chain from the raw measurements to the resulting tracks is formulated probabilistically. The presented approach is evaluated on experimental data and it is demonstrated that the data-driven measurement model outperforms a manually designed model.

==> stateOfTheArt.tex <==
\section{State of the Art}\label{s:sota}
In the following, existing work that is relevant to radar tracking and the different parts of the presented approach is briefly summarized. A more detailed review of multi-object tracking algorithms can be found in \cite{Vo.2015}. An elaborate overview of filters, measurement models, and applications of extended object tracking is given in \cite{Granstrom.2017}.

\subsection{Multi-Object Tracking}
Mutli-object tracking approaches estimate the state of multiple objects given a set of measurements that either originate from the objects or are clutter measurements, e.g. caused by sensor noise. In such problems, one of the greatest challenges is the measurement-to-object association that determines which object is updated with which measurement.

\Gls{PDA} filters such as the \gls{JPDA} filter \cite{Fortmann.1983} or the \gls{JIPDA} filter \cite{Musicki.2004} determine association probabilities for each measurement and compute weighted updates using all matching measurements. In contrast, \gls{MHT} approaches construct different association hypotheses which are evaluated and propagated to the future. As soon as new measurements are able to resolve the uncertainty in previous association decisions, false hypotheses are discarded which leads to a deferred decision logic \cite{Blackman.2004}.

Another group of multi-object tracking approaches is based on \gls{FISST} \cite{Mahler.2004,Mahler.2007}. \gls{FISST} is a rather recent theoretical framework which aims at providing a rigorous Bayesian formulation of the multi-object problem and mathematical tools which allow to derive different filter algorithms. These include \gls{PHD} filters \cite{Mahler.2007b} which constitute a first-order moment approximation of the multi-object estimation problem or the recently developed \gls{GLMB} \cite{Vo.2013} and \gls{LMB} \cite{Reuter.2014} filters which are based on specific types of multi-object distributions that allow for closed form solutions. While the original versions of these filters still assume that each object either gives rise to a single measurement or is misdetected, extensions to the extended object case have been presented in \cite{Mahler.2009} and \cite{Beard.2016}, respectively.

\subsection{Radar Data Processing and Measurement Models}\label{s:radarMeasModels}
\subsubsection{Preprocessing Routines} There are different examples for preprocessing routines that reduce multiple radar detections to meta-measurements that can then be used in classical point tracking approaches. For instance, \cite{Roos.2016} and \cite{Schlichenmaier.2017} present approaches to fit L-shapes and bounding boxes to high-resolution radar measurements from vehicles. In \cite{Dickmann.2015} and \cite{Elfring.2016}, clustering multiple detections and selecting different reference points from the clusters are part of the processing chain. Using the \gls{EM} algorithm, a set of reflection points is fitted to radar data in \cite{Bordonaro.2015} to obtain an intermediate state estimate of a plane. \cite{Kellner.2013b} extracts the vehicle speed directly from multiple measurements by fitting velocity profiles to the data. Incorporating a second sensor additionally allows for determining the yaw rate \cite{Kellner.2014} and \cite{Kellner.2016} demonstrates how to incorporate the extracted information in a tracking algorithm.

\subsubsection{Point Tracking Considering the Extent} In \cite{Kim.2015}, the vehicle extent is taken into account by assuming a rectangular shape and that the measurement originates from one of twelve specific points on the rectangle. As only one measurement is processed at each time step, however, this approach is not an extended object approach as defined in \cite{Granstrom.2017}.

\subsubsection{Extended Object Models} Extended object measurement models can be grouped according to different modeling paradigms \cite{Granstrom.2017}. One approach is to model objects as a set measurement sources with specific spatial structure, see for example \cite{Salmond.1999}. In \cite{Darms.2009} vehicles are modeled as rectangles and multiple radar measurements may be associated to different sources on the rectangle corners and surfaces centers. Another approach which uses typical radar reflection centers, e.g. wheel houses, is presented in \cite{Gunnarsson.2007} and \cite{Hammarstrand.2012}. An extension of this method which estimates the number of reflection centers and their location is proposed in \cite{Hammarstrand.2012b}.

A second variant of extended object models defines spatial distributions for the location of the measurement as initially proposed in \cite{Gilholm.2005b} and \cite{Gilholm.2005c}. Prominent examples are the random matrix model which assumes an elliptical shape \cite{Koch.2008}, or the \gls{RHM} \cite{Baum.2014} and Gaussian process model \cite{Wahlstroem.2015} which allow for the estimation of arbitrary star-convex shapes. For radar tracking, the random matrix model has been extended to incorporate Doppler measurements in \cite{Schuster.2015}. However, the variation of the expected Doppler measurements over the entire object extent due to the measurement angle or yaw rate is not considered. A polynomial object model for tracking stationary objects such as guard rails with radar sensors was presented in \cite{Lundquist.2010}. Recently, a Volcanormal density, which could be integrated in an extended object filter, has been proposed as vehicle model in \cite{Broeit.2017}. It assumes an elliptical shape and that measurements are more likely on the vehicle surface. An additional component is added to the model to incorporate Doppler measurements.

A third paradigm for extended object models is to chose a physics-based approach \cite{Granstrom.2017}. Although many of the aforementioned approaches (e.g. \cite{Hammarstrand.2012}) are certainly based on physical models and may as well be assigned to this category, it is used here to introduce two approaches based on ray tracing. In \cite{Adam.2013}, the rear surface of the tracked vehicle is modeled as stick and expected locations of measurements are determined by intersecting radar beams with the stick. In contrast, the direct scattering model from \cite{Knill.2016} uses a full rectangular description of the vehicle and allows for tracking vehicles in arbitrary maneuvers with arbitrary aspect angles. It was incorporated into a multi-object framework in \cite{Scheel.2016a}.

\subsection{Radar Models for Simulation}
In addition to the mentioned sensor models for object tracking, there exists work on models for sensor simulation. Examples are \cite{Schuler.2008} which presented an approach for obtaining a simplified vehicle representation in terms of reflection centers from ray tracing simulations or\cite{Buhren.2006} which has led to the development of the measurement models in \cite{Gunnarsson.2007,Hammarstrand.2012,Hammarstrand.2012b}.

In contrast to such simulation models on the basis of expert knowledge or physical calculations, methods that use machine learning techniques and obtain models directly from measured data have been developed. For instance, \cite{Wheeler.2017} uses deep neural networks to simulate a radar grid of power values from the inputs of a spatial raster that describes the nature of the ground and an object list. A statistical study on the relation of measurement locations in dependence on the aspect angle is provided in \cite{Berthold.2017}. In \cite{Hirsenkorn.2015} and \cite{Hirsenkorn.2016} kernel density estimation methods are employed to generate a conditional density of the position of radar object detections given the actual object state.
